The State and Fate of Linguistic Diversity and Inclusion in the NLP World

Language technologies contribute to promoting multilingualism and linguistic diversity around the world. However, only a very small number of the over 7000 languages of the world are represented in the rapidly evolving language technologies and applications. In this paper we look at the relation between the types of languages, resources, and their representation in NLP conferences to understand the trajectory that different languages have followed over time. Our quantitative investigation underlines the disparity between languages, especially in terms of their resources, and calls into question the "language agnostic" status of current models and systems. Through this paper, we attempt to convince the ACL community to prioritise the resolution of the predicaments highlighted here, so that no language is left behind.

==> sections/5_embeddings.tex <==
\section{Entity Embeddings}

The pure statistical measures discussed in the previous section signal at variance in acceptance of different languages at different NLP venues across time. However, there are usually multiple subtle factors which vanilla statistics fail to capture. Embeddings, on the other hand, have been found extensively useful in NLP tasks as they are able to learn relevant signals directly from the data and uncover these rather complex nuances. To this end, we propose an approach to jointly learn the representations of conferences, authors and languages. Our primary motivation to learn these embeddings is to understand if there are any non-trivial patterns available in the ACL Anthology discussed in the previous section, and use these trends to answer our research questions.

% The pure statistical measures discussed in the previous section signal at variance in acceptance of different languages at different NLP venues across time. However, there are usually multiple subtle factors which vanilla statistics fail to capture. Embeddings, on the other hand, have been found extensively useful in NLP tasks are they are able to learn relevant signals directly from the data and uncover these rather complex nuances. To this end, we propose an approach to jointly learn the representations of conferences, authors and languages. Our primary motivation to learn these embeddings is to understand if there are any non-trivial patterns available in the ACL Anthology dataset discussed in the previous section, and use these trends to answer our research questions.


\subsection{Model}
% To jointly learn the embeddings of conferences, authors and languages, we propose an approach similar to Word2Vec \citep{word2vec}. In Word2Vec (skipgram formulation), the task of the model is that given the target word, predict `K' words to the left and `K' words to the right of that word. So effectively, the target word is the input and the words to the left or right to that word are the outputs. This type of a learning task tries to create embeddings for the words which co-occur together in the same context. 
% Inspired by the learning setting of Word2Vec \citep{word2vec}, we define the following model to learn the embedding of a conference/author/language (aka entity) such that entity which have similar word distributions should co-occur together. For example, in case of an author `A', who works extensively on language `L' and publishes at conference `C', then the embeddings of `A', `L' and `C' should be close to each other. 

Inspired by the learning setting of Word2Vec \citep{word2vec}, we define the following model to jointly learn the embeddings of entities (conference/author/language) such that entities which have similar contextual distributions should co-occur together. For example, in case of an author `A', who works extensively on language `L' and publishes at conference `C', the embeddings of `A', `L' and `C' should be close to each other. 

%In order learn these embeddings, we use a single hidden layer neural network such given a paper, its authors, its conference, and the languages mentioned in it, the model's task is to randomly predict the words written in this paper. We only take the title and abstract from the paper in this learning as they provide a more concise signal without noise. 

\begin{figure}
    \centering
    \includegraphics[width=0.35\textwidth]{images/EntityEmbeddings.pdf}
    \caption{Model architecture to learn entity embeddings}
    \label{fig:model}
\end{figure}

Figure \ref{fig:model} shows an outline of the model. The input layer corresponds to the entities and is of the size of number of entities in the entire dataset. Hidden layer is the size of the embedding dimension that is desired. The output layer is for the output words and is of the size of the vocabulary to enable prediction of words for the input entity. $W_{HL-E}$ is the weight matrix from input layer (Entity layer) to the hidden layer, and $W_{V-HL}$ is the weight matrix for the hidden layer to output layer computation. At the end of training, $W_{HL-E}$ is the matrix containing embeddings of entities and $W_{V-HL}$ is the matrix containing the embeddings of words. To train the model, a single entity of a paper is given as input, and the model is asked to predict the words from the title and abstract of the paper. The entities we are learning in this setting are - authors of the paper, languages mentioned in the paper, conference where the paper was accepted (e.g. ACL), and, conference and year together (e.g. ACL\_2019)\footnote{We remove collisions due to author names by ACL Anthology ids.}. %Through this embedding technique, we aim to bring together entities which are related to similar papers closer in the embedding space; addition of both conference and, conference and year helps the model to learn a single vector for each conference as well a separate vector for the respective for a given year. 

Our model has same hyperparameters as that of Word2Vec. To determine the optimal hyper-parameters for  the model, we take the entire dataset and split it into a 80-20 ratio, and given the embedding of a paper, the task is to predict the year in which the paper is published. Given this vector for a paper, we use a linear regression model such that given this vector, the model is supposed to predict the year in which the paper was published. We measured both $R^2$ measure of variance in regression and mean absolute error (MAE). $R^2$ is usually in the range of 0 to 1.00 (or 0 to 100\%) where 1.00 is considered to be the best. MAE has no upper bound but the smaller it is the better, and 0 is its ideal value. We observed that our model does not show significant difference across any hyperparaeters except for the size of embeddings. The best dimension size for our embeddings is 75, and, we observed the corresponding $R^2$ value of 0.6 and an MAE value of 4.04.

\begin{table}[]
\small
\begin{tabular}{@{}lllll@{}}
\toprule
Class & MRR(5)  & MRR(10) & MRR(15) & MRR(20) \\ \midrule
0     & 0.72281 & 0.69146 & 0.63852 & 0.57441 \\
1     & 0.57210 & 0.52585 & 0.45354 & 0.40904 \\
2     & 0.47039 & 0.45265 & 0.41521 & 0.38157 \\
3     & 0.59838 & 0.52670 & 0.45131 & 0.42899 \\
4     & 0.56016 & 0.47795 & 0.51199 & 0.50681 \\
5     & 0.56548 & 0.51471 & 0.54326 & 0.47619\\ \bottomrule
\end{tabular}
\caption{MRR of Class of Languages}
\label{MRR_Embeddings}
\end{table}

%Our model has same hyperparameters as that of Word2Vec. To determine the optimal hyper-parameters for  the model, we take the entire dataset and split it into a 80-20 ratio, and given the embedding of a paper, the task is to predict the year in which the paper is published. Using the 80\% split, we first train the above model. To compute the embedding of a paper, we consider it as an entity and ask the model to predict the words from its title and abstract similar to the training, but this paper was not seen in training. Given this vector for a paper, we use a linear regression model such that given this vector, the model is supposed to predict the year in which the paper was published. We measured both $R^2$ measure of variance in regression and mean absolute error (MAE). $R^2$ is usually in the range of 0 to 1.00 (or 0 to 100\%) where 1.00 is considered to be the best. MAE has no upper bound but the smaller it is the better, and 0 is the ideal value for the model.

%We tuned our model on window size (i.e. number of words to be predicted from the document) (from 3 to 7, step size = 1), negative subsampling (similar to Word2Vec, from 5 to 8, step size = 1) and dimensions of hidden layer (50, 75, 100, 150, 200). Our experiments showed that dimension size of 75 is optimal but window size and negative subsampling do not considerably impact the performance. Hence, we choose the value of 5 for window size and 5 for negative subsampling. At these hyper-parameters, we observed an $R^2$ value of 0.6 and an MAE value of 4.04.

\begin{figure*}
    \centering
    \includegraphics[scale=0.4]{images/ACL_V2.JPG}
    \caption{t-SNE visualization of the learnt conference and language embeddings}
    \label{t-sne-conf}
\end{figure*}

%\subsection{Test}
\subsection{Method}
The output of the entity embedding model gave us trained embeddings for each author in the corpus, conference (e.g. ACL), conference and year (e.g. ACL\_2019), and languages mentioned in the paper. We projected these embeddings into 2 dimensions using t-SNE \citep{t-SNE}. Figure \ref{t-sne-conf} shows the 2-D projections for  conferences. For the sake of clarity, we only plotted ACL, LREC, Workshops and CL among the conferences, and all languages from the taxonomy, except languages in category 0.  Through these conference and languages vectors, we wanted to also understand how close conferences are to the languages. From Figure \ref{t-sne-conf}, we can see that languages are somewhat below the conferences are closer to some conferences while distant from others. To quantify this analysis, we compute the cosine distance between the conference vector and the mean of the vector each category of the taxonomy. Table \ref{distance_vectors} shows the cosine distance between the conferences and the each category of languages.

Moreover, to analyze the role of an individual author and a community for each language category, we computed variation of Mean Reciprocal Rank (MRR). We consider a language `L', and we take the `K' closest authors to `L' using cosine distance, and then take the closest `M' languages to each author. If `L' is present in the closest languages of an author, then we take the rank of `L' in that list, inverse it, and average it for the `K' authors. To compute this metric for a class of languages from the taxonomy, we take the mean of the MRR for all languages in that class. Table \ref{MRR_Embeddings} shows the MRR of various categories of languages. 



\begin{table}
\small
\begin{tabular}{@{}lllllll@{}}
\toprule
Conf/Class         & \textbf{0} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} \\ \midrule
\textbf{LREC}      & 0.505    & 0.514    & 0.522     & 0.419    & 0.356    & 0.323    \\
\textbf{Workshops} & 0.501    & 0.546    & 0.533    & 0.404    & 0.281    & 0.207    \\
\textbf{CONLL}     & 0.542    & 0.598    & 0.634    & 0.491     & 0.395    & 0.455    \\
\textbf{EACL}      & 0.532    & 0.547     & 0.587     & 0.451    & 0.341    & 0.316     \\
\textbf{ACL}       & 0.480    & 0.505   & 0.600    & 0.422     & 0.337    & 0.291    \\
\textbf{TACL}      & 0.522    & 0.556    & 0.658    & 0.482    & 0.376    & 0.465    \\
\textbf{CL}        & 0.669    & 0.783    & 0.799    & 0.746    & 0.652    & 0.593    \\
\textbf{NAACL}     & 0.477    & 0.517    & 0.589    & 0.467    & 0.387    & 0.333    \\
\textbf{COLING}    & 0.483    & 0.528    & 0.552    & 0.461    & 0.373    & 0.304    \\
\textbf{EMNLP}     & 0.566    & 0.589    & 0.660    & 0.512    & 0.463    & 0.446   \\ \bottomrule
\end{tabular}
\caption{Distance between conference vectors and mean class vectors of languages}
\label{distance_vectors}
\end{table}

%\begin{table*}[!t]
%\small
%\begin{tabular}{@{}lllllllllll@{}}
%\toprule
%Class & LREC & WS & CONLL & EACL & ACL & TACL & CL & NAACL & COLING & EMNLP\\ \midrule
%0 & 0.505667 & 0.501478 & 0.542069 & 0.532920 & 0.480057 & 0.521693 & 0.669239 & 0.477215 & 0.483270 & 0.566253\\
%1 & 0.514077 & 0.546556 & 0.598566 & 0.547302 & 0.504767 & 0.555851 & 0.782559 & 0.516846 & 0.527981 & 0.588785\\
%2 & 0.522202 & 0.533760 & 0.634278 & 0.587701 & 0.600340 & 0.657836 & 0.799324 & 0.589349 & 0.552471 & 0.659754\\
%3 & 0.419882 & 0.404691 & 0.491904 & 0.451078 & 0.421598 & 0.482064 & 0.745634 & 0.467465 & 0.460928 & 0.519606\\
%4 & 0.356744 & 0.281469 & 0.395685 & 0.340791 & 0.337215 & 0.376109 & 0.652010 & 0.387023 & 0.373515 & 0.463028\\
%5 & 0.323976 & 0.207775 & 0.455164 & 0.315802 & 0.291207 & 0.464676 & 0.592889 & 0.333119 & 0.303659 & 0.446172
%\\\bottomrule
%\end{tabular}
%\caption{Distance between conference vectors and mean class vectors of languages}
%\label{distance_vectors}
%\end{table*}





\subsection{Findings}



\textbf{Time waits for no conference}: Considering ACL as the premier conference in NLP, we can see that there is a left to right trend in the graph such that with ACL in 1983 in the left, and year gradually increases as we move towards the right with ACL 2019.EACL, NAACL, EMNLP, CONNL, TACL, and COLING follow the same trend that as we move from left to right, year increase for these respective conferences. We can say that the axis represents the progression to time to a certain extent, or it may even be a representation of a shift in technology in NLP, moving from theoretical research focused on grammar and formalism on the left to a data-driven, more ML-oriented approach on the right. Interestingly, we can see that the embeddings of most of the CL editions are positioned on the left, which makes sense that CL has a research focus on methods involving statistical algorithms and grammar formalism, and less on heavily data-driven methods. \\
\textbf{Long distance relationships?}: From Figure \ref{t-sne-conf}, we can note that the less-resourced language classes are farther away from the trend-line of ACL than the more resourced ones, with class 5 being the closest, and finally till class 1. However, as Class 0 languages are large in number, these were scattered in the projection as they are rarely mentioned in conferences, they are scattered around the visualization (not shown). Table \ref{distance_vectors} also shows a very similar trend that while ACL is an at average distance of 0.291 from category 5 languages, its almost more than double far away from category 2. There is also a very steep rise in distance of the ACL vector from category 4 to category 3. In fact, similar trends are visible for other ACL related conferences including EACL, NAACL, EMNLP and TACL. \\
\textbf{Closer than most}: Again, as previous analyses have shown us, LREC and Workshop embeddings are closer to the language embeddings as compared to the other conferences as shown in Figure \ref{t-sne-conf}. We can see that in Table \ref{distance_vectors} workshops and LREC are closest from category 2 to category 5 whereas almost all conferences are somewhat at the same distance from category, except the CL journal. The trend for category 0 languages seems somewhat different than the usual trend is this table, probably because of the large number of languages in this category as well as the sparsity in papers. \\
%Moreover, in the trend for ACL, EACL, and, NAACL there is a rather steep increase in distance between category 3 and category 4 indicating that while these conferences are closer to categories 4 and 5, they are uniformly distant in the embedding space from the languages in other categories.\\
\textbf{Some heroes don't wear capes}: 
Table \ref{MRR_Embeddings} shows the MRR for each class of languages in the taxonomy, where MRR(K) indicates that the closest `K' authors were considered. We fixed the number of languages for each author to be 20, so as to understand the impact of the community when the number of languages remains unchanged. A higher value of this measure indicates a focused community working on that particular language. From Table \ref{MRR_Embeddings}, it can be seen that class 0 has the highest MRR across different K values. This shows that perhaps low resources languages have some research groups solely focus on the challenges related to them. The trend of MRR from class 0 to class 5 shows a decreasing trend, except for class 2, thereby indicating that more popular languages are addressed by more number of authors.
%Hence, we can establish that time is somewhat representative of time. Considering ACL as the central piece of our plot, and we computed Pearson's correlation coefficient with X-coordinate of ACL conference vectors and their corresponding years, the value is 0.98. We believe that the Y-coordinate is composite and captures other aspects of the dataset. This result, however, is non-trivial since workshops, LREC and CL journal do not follow this trend. 



 


%\subsection{Understanding role of research community in the linguistic resource divide}
%An important challenge in understanding where the low resources languages are lacking behind is to look at their contributors and research community. In this section of the paper, we want to understand whether for a certain category of languages in the taxonomy there is a focused community which works on them versus languages for which there are plenty of resources and datasets and are popular in the research community.

%To understand this aspect among the languages in the taxonomy, we compute a variation of Mean Reciprocal Rank (MRR) 

%Table \ref{MRR_Embeddings} shows the MRR for each class of languages in the taxonomy, where MRR(K) indicates that the closest `K' authors were considered. We fixed the number of languages for each author to be 20, so as to understand the impact of the community when the number of languages remains unchanged. A higher value of this measure indicates a focused community working on that particular language. From the table, it can be seen that class 0 has the highest MRR across different K values. This shows that perhaps low resources languages have some research groups solely focus on the challenges related to them. The trend of MRR from  class 0 to class 5 shows a decreasing trend, except for class 2, thereby indicating that more popular languages are addressed by more number of authors. 





%\subsection{Findings}
%\textbf{Time waits for no conference}: There is a clear trend of conferences such as ACL, EMNLP, NAACL, COLING moving from left to right from older to newer iterations of the conferences. We can say that the axis represents the progression to time to a certain extent, or it may even be a representation of a shift in technology in NLP, moving from theoretical research focused on grammar and formalism on the left to a data-driven, more ML-oriented approach on the right. Interestingly, we can see that the embeddings of most of the CL editions are positioned on the left, which makes sense that CL has a research focus on methods involving statistical algorithms and grammar formalisms, and less on heavily data-driven methods. \\
%\textbf{Losing distance}: We can note that the less-resourced language classes are farther away from the trend-line of ACL,EMNLP, and NAACL than the more resourced ones, with class 5 being the closest, and finally till class 1. However, as Class 0 languages are large in number and didn't have a strong enough signal for projection as they are rarely mentioned in conferences, they are scattered around the visualization (not shown). \\
%\textbf{Closer than most}: Again, as previous analyses have shown us, LREC and Workshop embeddings are closer to the language embeddings as compared to the other conferences. In fact, LREC forms a distinct cluster, which could indicate that they have a similar underlying research mission through iterations.\\
%\textbf{Some heroes don't wear capes}: From Table \ref{MRR_Embeddings}, it can be seen that class 0 has the highest MRR across different K values. This shows that perhaps low resources languages have some research groups solely focus on the challenges related to them. The trend of MRR from  class 0 to class 5 shows a decreasing trend, except for class 2, thereby indicating that more popular languages are addressed by more number of authors.

==> sections/5_embeddings_v2.tex <==
\section{Entity Embeddings}

The pure statistical measures discussed in the previous section signal at variance in acceptance of different languages at different NLP venues across time. However, there are usually multiple subtle factors which vanilla statistics fail to capture. Embeddings, on the other hand, have been found extensively useful in NLP tasks as they are able to learn relevant signals directly from the data and uncover these rather complex nuances. To this end, we propose an unique approach to jointly learn the representations of conferences, authors and languages, which we collectively term as entities. The proposed embedding method allows us to project these entities in the same space enabling us to effectively compute the distance between conferences, and languages, and uncover patterns about the research community of a language.

% The pure statistical measures discussed in the previous section signal at variance in acceptance of different languages at different NLP venues across time. However, there are usually multiple subtle factors which vanilla statistics fail to capture. Embeddings, on the other hand, have been found extensively useful in NLP tasks are they are able to learn relevant signals directly from the data and uncover these rather complex nuances. To this end, we propose an approach to jointly learn the representations of conferences, authors and languages. Our primary motivation to learn these embeddings is to understand if there are any non-trivial patterns available in the ACL Anthology dataset discussed in the previous section, and use these trends to answer our research questions.


\subsection{Model}
% To jointly learn the embeddings of conferences, authors and languages, we propose an approach similar to Word2Vec \cite{word2vec}. In Word2Vec (skipgram formulation), the task of the model is that given the target word, predict `K' words to the left and `K' words to the right of that word. So effectively, the target word is the input and the words to the left or right to that word are the outputs. This type of a learning task tries to create embeddings for the words which co-occur together in the same context. 
% Inspired by the learning setting of Word2Vec \cite{word2vec}, we define the following model to learn the embedding of a conference/author/language (aka entity) such that entity which have similar word distributions should co-occur together. For example, in case of an author `A', who works extensively on language `L' and publishes at conference `C', then the embeddings of `A', `L' and `C' should be close to each other. 

Inspired by the learning setting of Word2Vec \cite{mikolov2013efficient}, we define the following model to jointly learn the embeddings of entities (conference/author/language) such that entities which have similar contextual distributions should co-occur together. For example, for an author {\bf A}, who works more extensively on language {\bf $L_{i}$} than {\bf $L_{j}$} and publishes more at conference {\bf $C_{m}$} than at conference {\bf $C_{n}$}, the embeddings of {\bf A} would be closer {\bf $L_{i}$} than {\bf $L_{j}$} and {\bf $C_{m}$}  than {\bf $C_{n}$}.

The learning task of the model is given an entity (conference, author or language) and a paper associated with the entity, the model is asked to predict $K$ randomly sampled words from the title and the abstract of the paper. We only take the title and abstract from the paper for our learning task as they provide a more concise signal without noise. This model draws parallels to the Skipgram model of Word2Vec (where given an input word in Skipgram model, the task is to predict the context around the word) - where the input word in Skipgram is equivalent to the input entity and $K$ random words from the paper are equivalent to the context of the input word.

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{images/ARCH.png}
    \caption{Model architecture to learn entity embeddings}
    \label{fig:model}
\end{figure}


Figure \ref{fig:model} shows an outline of the model. The input layer corresponds to the entities and has size equal to the total number of entities in the dataset. Hidden layer size is the same as the desired embedding dimension. The output layer predicts words for the input entity and is of the same size as the vocabulary. $W_{E \times N}$ is the weight matrix from input layer (Entity layer) to the hidden layer, and $W_{N \times V}$ is the weight matrix for the hidden layer to output layer computation. At the end of training, $W_{E \times N}$ is the matrix containing embeddings of entities and $W_{N \times V}$ is the matrix containing the embeddings of words. To train the model, a single entity of a paper is given as input, and the model is asked to predict the words from the title and abstract of the paper. The entities we are learning are - authors of the paper, languages mentioned in the paper, conference where the paper was accepted (e.g. \confacl), and the conference iteration (e.g. acl\_2019). We describe the model detail and hyperparameter tuning in appendix.  %Through this embedding technique, we aim to bring together entities which are related to similar papers closer in the embedding space; addition of both conference and, conference and year helps the model to learn a single vector for each conference as well a separate vector for the respective for a given year. 

% \footnote{We remove collisions due to author names by ACL Anthology ids.}

The goal of the model is to maximize probability of predicting the random $K$ words, given the entity id as the input

\begin{equation}
    \frac{1}{M}  \frac{1}{K} \sum_{m=1}^{M} \sum_{k=1}^{K} \sum_{i=1}^{I} \textit{p}(w_{i} | E_{<i,P_{j}>})
\end{equation}

where $E_{<i,P_{j}>}$ is the entity $E_{i}$ which is associated with the ${P_{j}}^{th}$ paper and $\textit{p}$ is the probability of predicting the word $w_{i}$ out of the $K$ words sampled from the paper and $M$ is the total number of papers in the dataset.
 
In order to maximize this probability, we train the model to optimize the cross entropy loss similar to Word2Vec \cite{mikolov2013efficient}, including the negative subsampling strategy. 

\begin{table}[!ht]
\small
{\renewcommand{\arraystretch}{\pad}
\begin{tabular}{! \vbl >{\columncolor[HTML]{EFEFEF}}P{0.6cm}|P{1.2cm}|P{1.2cm}|P{1.2cm}|P{1.2cm}! \vbl}
\hbl
\cellcolor[HTML]{C0C0C0}\textbf{Class} & \cellcolor[HTML]{EFEFEF}\textbf{MRR(5)}  & \cellcolor[HTML]{EFEFEF}\textbf{MRR(10)} & \cellcolor[HTML]{EFEFEF}\textbf{MRR(15)} & \cellcolor[HTML]{EFEFEF}\textbf{MRR(20)} \\\hline
0     & \mrr{0.72281} & \mrr{0.69146} & \mrr{0.63852} & \mrr{0.57441} \\\hline
1     & \mrr{0.57210} & \mrr{0.52585} & \mrr{0.45354} & \mrr{0.40904} \\\hline
2     & \mrr{0.47039} & \mrr{0.45265} & \mrr{0.41521} & \mrr{0.38157} \\\hline
3     & \mrr{0.59838} & \mrr{0.52670} & \mrr{0.45131} & \mrr{0.42899} \\\hline
4     & \mrr{0.56016} & \mrr{0.47795} & \mrr{0.51199} & \mrr{0.50681} \\\hline
5     & \mrr{0.56548} & \mrr{0.51471} & \mrr{0.54326} & \mrr{0.47619}\\\hbl
\end{tabular}}
\caption{Language-Author-Language MRR on Taxonomy Classes}
\label{MRR_Embeddings}
\end{table}

%Our model has same hyperparameters as that of Word2Vec. To determine the optimal hyper-parameters for  the model, we take the entire dataset and split it into a 80-20 ratio, and given the embedding of a paper, the task is to predict the year in which the paper is published. Using the 80\% split, we first train the above model. To compute the embedding of a paper, we consider it as an entity and ask the model to predict the words from its title and abstract similar to the training, but this paper was not seen in training. Given this vector for a paper, we use a linear regression model such that given this vector, the model is supposed to predict the year in which the paper was published. We measured both $R^2$ measure of variance in regression and mean absolute error (MAE). $R^2$ is usually in the range of 0 to 1.00 (or 0 to 100\%) where 1.00 is considered to be the best. MAE has no upper bound but the smaller it is the better, and 0 is the ideal value for the model.

%We tuned our model on window size (i.e. number of words to be predicted from the document) (from 3 to 7, step size = 1), negative subsampling (similar to Word2Vec, from 5 to 8, step size = 1) and dimensions of hidden layer (50, 75, 100, 150, 200). Our experiments showed that dimension size of 75 is optimal but window size and negative subsampling do not considerably impact the performance. Hence, we choose the value of 5 for window size and 5 for negative subsampling. At these hyper-parameters, we observed an $R^2$ value of 0.6 and an MAE value of 4.04.

\begin{figure*}
    \centering
    \includegraphics[scale=0.4]{images/embeddings_final.png}
    \caption{t-SNE visualization of the learnt conference and language embeddings}
    \label{t-sne-conf}
\end{figure*}

%\subsection{Test}
\subsection{Method}
The output of the entity embedding model gave us trained embeddings for each author in the corpus, conference (e.g. \confacl), conference and year (e.g. acl\_2019), and languages mentioned in the paper. We projected these embeddings into 2 dimensions using t-SNE \cite{maaten2008visualizing}. Figure \ref{t-sne-conf} shows the 2-D projections for  conferences. For the sake of clarity, we only plotted \confacl, \conflrec, \confws and \confcl among the conferences, and all languages from the taxonomy, except languages in class 0.  Through this plot, we wanted to understand how languages are represented at different venues.

%how close conferences are to the languages. From Figure \ref{t-sne-conf}, we can see that languages are somewhat below the conferences are closer to some conferences while distant from others. 

%To quantify this analysis, we compute the cosine distance between the conference vector and the mean of the vector each category of the taxonomy. Table \ref{distance_vectors} shows the cosine distance between the conferences and the each category of languages.


%In order to understand, how 
Moreover, to analyze the role of an individual author and a community for each language class, we computed a variation of Mean Reciprocal Rank (MRR). We consider a language {\bf L}, and we take the {\bf K} closest authors to {\bf L} using cosine distance, and then take the closest {\bf M} languages to each author. If {\bf L} is present in the closest languages of an author, then we take the rank of {\bf L} in that list, inverse it, and average it for the {\bf K} authors. To compute this metric for a class of languages from the taxonomy, we take the mean of the MRR for all languages in that class. Table \ref{MRR_Embeddings} shows the MRR of various class of languages. 



%\begin{table}
%\small
%\begin{tabular}{@{}lllllll@{}}
%\toprule
%Conf/Class         & \textbf{0} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} \\ \midrule
%\textbf{\conflrec}      & 0.505    & 0.514    & 0.522     & 0.419    & 0.356    & 0.323    \\
%\textbf{\confws} & 0.501    & 0.546    & 0.533    & 0.404    & 0.281    & 0.207    \\
%\textbf{\confconll}     & 0.542    & 0.598    & 0.634    & 0.491     & 0.395    & 0.455    \\
%\textbf{\confeacl}      & 0.532    & 0.547     & 0.587     & 0.451    & 0.341    & 0.316     \\
%\textbf{\confacl}       & 0.480    & 0.505   & 0.600    & 0.422     & 0.337    & 0.291    \\
%\textbf{\conftacl}      & 0.522    & 0.556    & 0.658    & 0.482    & 0.376    & 0.465    \\
%\textbf{\confcl}        & 0.669    & 0.783    & 0.799    & 0.746    & 0.652    & 0.593    \\
%\textbf{\confnaacl}     & 0.477    & 0.517    & 0.589    & 0.467    & 0.387    & 0.333    \\
%\textbf{\confcoling}    & 0.483    & 0.528    & 0.552    & 0.461    & 0.373    & 0.304    \\
%\textbf{\confemnlp}     & 0.566    & 0.589    & 0.660    & 0.512    & 0.463    & 0.446   \\ %\bottomrule
%\end{tabular}
%\caption{Distance between conference vectors and mean class vectors of languages}
%\label{distance_vectors}
%\end{table}

%\begin{table*}[!t]
%\small
%\begin{tabular}{@{}lllllllllll@{}}
%\toprule
%Class & \conflrec & WS & \confconll & \confeacl & \confacl & \conftacl & \confcl & \confnaacl & \confcoling & \confemnlp\\ \midrule
%0 & 0.505667 & 0.501478 & 0.542069 & 0.532920 & 0.480057 & 0.521693 & 0.669239 & 0.477215 & 0.483270 & 0.566253\\
%1 & 0.514077 & 0.546556 & 0.598566 & 0.547302 & 0.504767 & 0.555851 & 0.782559 & 0.516846 & 0.527981 & 0.588785\\
%2 & 0.522202 & 0.533760 & 0.634278 & 0.587701 & 0.600340 & 0.657836 & 0.799324 & 0.589349 & 0.552471 & 0.659754\\
%3 & 0.419882 & 0.404691 & 0.491904 & 0.451078 & 0.421598 & 0.482064 & 0.745634 & 0.467465 & 0.460928 & 0.519606\\
%4 & 0.356744 & 0.281469 & 0.395685 & 0.340791 & 0.337215 & 0.376109 & 0.652010 & 0.387023 & 0.373515 & 0.463028\\
%5 & 0.323976 & 0.207775 & 0.455164 & 0.315802 & 0.291207 & 0.464676 & 0.592889 & 0.333119 & 0.303659 & 0.446172
%\\\bottomrule
%\end{tabular}
%\caption{Distance between conference vectors and mean class vectors of languages}
%\label{distance_vectors}
%\end{table*}





\subsection{Findings}



$\bullet$ \textbf{Time waits for no conference}: We can see a left to right trend in Figure \ref{t-sne-conf} with \confacl in 1983 in the left, and subsequent iterations laid out as we go right. \confeacl, \confnaacl, \confemnlp, \confconll, \conftacl, and \confcoling follow the same trend that as we move from left to right (not shown for clarity), year increase for these respective conferences. We can say that the axis represents the progression of time to a certain extent, or it may even be a representation of a shift in technology in NLP, moving from theoretical research focused on grammar and formalisms on the left to a data-driven, more ML-oriented approach on the right. Interestingly, we can see that the embeddings of most of the \confcl editions are positioned on the left, which makes sense as \confcl given their research focus on statistical algorithms and grammar formalisms. \\
$\bullet$ \textbf{Long distance relationships?}: From Figure \ref{t-sne-conf}, we can note that the less-resourced language classes are farther away from the trend-line of \confacl than the more resourced ones, with class 5 being closest, and class 1 being farthest. However, as Class 0 languages are large in number, these were scattered in the projection as they are rarely mentioned in conferences, hence we omit their visualization. The visualization illustrates that languages are spreading out in semi-circular fashion from \confacl downwards with popular classes of taxonomy like class 5 and class 4 being closer while other spreading out farther. Again, as previous analyses have shown us, \conflrec and \confws embeddings are closer to the language embeddings as compared to the other conferences as shown in Figure \ref{t-sne-conf}. In fact, \conflrec cluster is right in the middle of language clusters and so is the major part of the \confws cluster.\\
%Moreover, in the trend for \confacl, \confeacl, and, \confnaacl there is a rather steep increase in distance between category 3 and category 4 indicating that while these conferences are closer to categories 4 and 5, they are uniformly distant in the embedding space from the languages in other categories.\\
$\bullet$ \textbf{Not all heroes wear capes}: 
Table \ref{MRR_Embeddings} shows the MRR for each class of languages in the taxonomy, where MRR({\bf K}) considers the closest {\bf K} authors. We fixed the number of languages for each author to be 20, so as to understand the impact of the community when the number of languages remains unchanged. A higher value of this measure indicates a focused community working on that particular language. From Table \ref{MRR_Embeddings}, it can be seen that class 0 has the highest MRR across different {\bf K} values. This shows that perhaps low resource languages have some research groups solely focused on the challenges related to them. The trend of MRR from class 0 to class 5 shows a decreasing trend, except for class 2, thereby indicating that more popular languages are addressed by more number of authors. We also observed that even though \LANG{Japanese}, \LANG{Mandarin}, \LANG{Turkish} and \LANG{Hindi} (MRR(10) $ >0.75$)) are part of class 5 and class 4 and have a lot of resources, their MRR is higher even compared to low resource languages in another classes indicating that these languages have focused research communities working on them. On the other end of the spectrum, we observe a lot of low resource languages like \textit{Burmese} (MRR(10) $ =0.02$), \LANG{Javanese} (MRR(10) $ =0.23$) and \LANG{Igbo} (MRR(10) $ =0.13$) which have millions of speakers but still have significantly low MRR values, potentially indicating that not a lot of attention is being given to them in the research community.
%Hence, we can establish that time is somewhat representative of time. Considering \confacl as the central piece of our plot, and we computed Pearson's correlation coefficient with X-coordinate of \confacl conference vectors and their corresponding years, the value is 0.98. We believe that the Y-coordinate is composite and captures other aspects of the dataset. This result, however, is non-trivial since workshops, \conflrec and \confcl journal do not follow this trend. 




%\subsection{Understanding role of research community in the linguistic resource divide}
%An important challenge in understanding where the low resources languages are lacking behind is to look at their contributors and research community. In this section of the paper, we want to understand whether for a certain category of languages in the taxonomy there is a focused community which works on them versus languages for which there are plenty of resources and datasets and are popular in the research community.

%To understand this aspect among the languages in the taxonomy, we compute a variation of Mean Reciprocal Rank (MRR) 

%Table \ref{MRR_Embeddings} shows the MRR for each class of languages in the taxonomy, where MRR(K) indicates that the closest `K' authors were considered. We fixed the number of languages for each author to be 20, so as to understand the impact of the community when the number of languages remains unchanged. A higher value of this measure indicates a focused community working on that particular language. From the table, it can be seen that class 0 has the highest MRR across different K values. This shows that perhaps low resources languages have some research groups solely focus on the challenges related to them. The trend of MRR from  class 0 to class 5 shows a decreasing trend, except for class 2, thereby indicating that more popular languages are addressed by more number of authors. 





%\subsection{Findings}
%\textbf{Time waits for no conference}: There is a clear trend of conferences such as \confacl, \confemnlp, \confnaacl, \confcoling moving from left to right from older to newer iterations of the conferences. We can say that the axis represents the progression to time to a certain extent, or it may even be a representation of a shift in technology in NLP, moving from theoretical research focused on grammar and formalism on the left to a data-driven, more ML-oriented approach on the right. Interestingly, we can see that the embeddings of most of the \confcl editions are positioned on the left, which makes sense that \confcl has a research focus on methods involving statistical algorithms and grammar formalisms, and less on heavily data-driven methods. \\
%\textbf{Losing distance}: We can note that the less-resourced language classes are farther away from the trend-line of \confacl,\confemnlp, and \confnaacl than the more resourced ones, with class 5 being the closest, and finally till class 1. However, as Class 0 languages are large in number and didn't have a strong enough signal for projection as they are rarely mentioned in conferences, they are scattered around the visualization (not shown). \\
%\textbf{Closer than most}: Again, as previous analyses have shown us, \conflrec and Workshop embeddings are closer to the language embeddings as compared to the other conferences. In fact, \conflrec forms a distinct cluster, which could indicate that they have a similar underlying research mission through iterations.\\
%\textbf{Some heroes don't wear capes}: From Table \ref{MRR_Embeddings}, it can be seen that class 0 has the highest MRR across different K values. This shows that perhaps low resources languages have some research groups solely focus on the challenges related to them. The trend of MRR from  class 0 to class 5 shows a decreasing trend, except for class 2, thereby indicating that more popular languages are addressed by more number of authors.

==> sections/9_erratum.tex <==
\section{Erratum}
We noted an error in Table \ref{tab:taxstats} in the `\#Speakers column', along with small miscalculations in `\% of Total Langs' column. The trends and takeaways in the paper are in fact more strongly described with the corrected details. The corrected table is as follows:

\begin{table*}[!t]
\begin{center}
\small
{\renewcommand{\arraystretch}{\pad}
\begin{tabular}{! \vbl >{\columncolor[HTML]{EFEFEF}}c|c|c|c|c! \vbl}

      \hbl
      \cellcolor[HTML]{C0C0C0}\textbf{Class} & \cellcolor[HTML]{EFEFEF}\textbf{5 Example Languages} & \cellcolor[HTML]{EFEFEF}\textbf{\#Langs} & \cellcolor[HTML]{EFEFEF}\textbf{\#Speakers} & \cellcolor[HTML]{EFEFEF}\textbf{\% of Total Langs} \\
      \hline
     0 & \LANG{Dahalo}, \LANG{Warlpiri}, \LANG{Popoloca}, \LANG{Wallisian}, \LANG{Bora} & 2191 & 1.0B & 88.17\% \\
      \hline
     1 & \LANG{Cherokee}, \LANG{Fijian}, \LANG{Greenlandic}, \LANG{Bhojpuri}, \LANG{Navajo} & 222 & 1.0B & 8.93\% \\
      \hline
     2 & \LANG{Zulu}, \LANG{Konkani}, \LANG{Lao}, \LANG{Maltese}, \LANG{Irish} & 19 & 300M & 0.76\% \\
      \hline
     3 & \LANG{Indonesian}, \LANG{Ukranian}, \LANG{Cebuano}, \LANG{Afrikaans}, \LANG{Hebrew} & 28 & 1.1B & 1.13\% \\
      \hline
     4 & \LANG{Russian}, \LANG{Hungarian}, \LANG{Vietnamese}, \LANG{Dutch}, \LANG{Korean} & 18 & 1.6B & 0.72\% \\
      \hline
     5 & \LANG{English}, \LANG{Spanish}, \LANG{German}, \LANG{Japanese}, \LANG{French} & 7 & 2.5B & 0.28\% \\
      \hbl

\end{tabular}}
\caption{Number of languages, number of speakers, and percentage of total languages for each language class.}
\label{tab:taxstats}
 \end{center}
\end{table*}

==> sections/contr.tex <==
1. First, we ask some relevant and pertinent questions regarding the state of language inclusion in the context of resources and research.
2. To answer these questions, we conduct a multi-pronged quantitative analysis by first defining a taxonomy over 2300+ languages in terms of language resource availability. We use this taxonomy to guide our further analyses.
3. We then look at the typological diversity of available resources and briefly look into the repercussions of omitting languages with specific typological features in terms of multilingual system performance.
4. Following this, we empirically investigate the representation of languages in various NLP conferences such as ACL,EMNLP,NAACL,LREC, and more, via particular statistical measures.
5. We also propose an embedding algorithm to learn embeddings for conferences, languages and authors. We use these embeddings to further augment our analysis of language inclusion at NLP venues, and the role research community plays in developing the language technologies for different languages.
